An Adaptive Algorithm for Learning with Unknown Distribution Drift

We develop and analyze a general technique for learning with an unknown distribution drift. Given a sequence of independent observations from the last $T$ steps of a drifting distribution, our algorithm agnostically learns a family of functions with respect to the current distribution at time $T$. Unlike previous work, our technique does not require prior knowledge about the magnitude of the drift. Instead, the algorithm adapts to the sample data. Without explicitly estimating the drift, the algorithm learns a family of functions with almost the same error as a learning algorithm that knows the magnitude of the drift in advance. Furthermore, since our algorithm adapts to the data, it can guarantee a better learning error than an algorithm that relies on loose bounds on the drift. We demonstrate the application of our technique in two fundamental learning scenarios: binary classification and linear regression.

==> saving-stuff-here.tex <==


\subsubsection{Agnostic Learning of Binary Families}
Let $\mathcal{F}$ be a family of binary functions with VC dimension $\nu$. We seek to find with minimum expected value $f^* = \argmin_{f \in \mathcal{F}} P_1(f)$. As a simple corollary of \Cref{thm:main}, we can obtain the following result.
\begin{corollary}
There exists an algorithm that observes $X_1,\ldots,X_n$, and it returns a value $\hat{r}$ such that if $\hat{f} = \argmin_{f  \in \mathcal{F}} \ep_{1:\hat{r}}(f)$, then with probability at least $1-\delta$ it holds
\begin{align*}
P_1(\hat{f}) - P_1(f^*) \lesssim  \min_{r \leq n} \left( \sqrt{\frac{\nu}{r}} +\lVert P_1 - \ep_{1:r} \rVert_{\mathcal{F}}   \right) \left( \log\log(\hat{r}) + \log(1/\delta) \right)
\end{align*}
\end{corollary}
It is instructive to compare this upper bound with previous work. If we assume an upper bound $\Delta$ to the drift at each step, i.e. $\lVert P_i -P_{i+1}\rVert \leq \Delta$ for any $i \leq n-1$, then there is an algorithm that uses this information and it outputs a function $\hat{f}$ such that with probability at least $9/10$, it holds that 
\begin{align*}
P_1(\hat{f}) - P_1(f^*)  \lesssim  (\Delta \nu)^{1/3}
\end{align*}
This algorithm presents major drawbacks, as it requires apriori knowledge of the upper bound $\Delta$, and the guarantees are given as a function of this upper bound.

On the other hand, since this assumption implies $\lVert P_1 - \ep_{1:\hat{r}}\rVert_{\mathcal{F}} \leq r\Delta$, we have that
\begin{align*}
\min_{r \leq n} \left( \sqrt{\frac{\nu}{r}} +\lVert P_1 - \ep_{1:\hat{r}} \rVert_{\mathcal{F}}   \right) \leq \min_{r \leq n}\left( \sqrt{\frac{\nu}{r}}{r} + r\Delta \right) = O( \sqrt[3]{\nu\Delta})
\end{align*}
Therefore, we can obtain at least a similar guarantee by invoking the above corollary. However, our algorithm does not require a knowledge apriori of $\Delta$, and most importantly it is adaptive: if the upper bound $\Delta$ is very loose, and in the extreme case the data is i.i.d., our algorithm exhibits a better performance. We also investigate the tightness of our upper bound. 

\begin{theorem}
Let $\nu \in \mathbb{N}$. Let $d_1,\ldots,d_n$ be any non-negative and non-decreasing sequence such that $d_n \leq 1/\nu$. 
For any class of binary functions $\mathcal{F}$ with VC dimension $\nu$, and any learning algorithm $\mathcal{A}$, there exists a sequence of distributions $P_1,\ldots,P_n$ such that $\lVert P_1 - P_{1:r} \rVert = d_r$ for any $r \leq n$, and
\begin{align*}
\Exp P_1(\hat{f}) - P_{1}(f^*) = \Omega\left( \min_{r \leq n}\left( \sqrt{\frac{\nu}{r}} + \lVert P_1 - P_{1:r} \rVert_{\mathcal{F}} \right)\right)
\end{align*}
where $\hat{f} \in \mathcal{F}$ is the function returned by $\mathcal{A}$.

\end{theorem}


\iffalse
\comment{
In some cases, as we saw in other papers, it is possible to show that among all possible algorithms $\mathcal{A}$ that output a distribution $P_{\mathcal{A}} \in \mathcal{P}$ given $Z_1,\ldots,Z_n$,  it holds that
\begin{align*}
  \min_{\mathcal{A}} \max_{P_1,\ldots,P_n} \Exp d\left( \theta(P_1), \theta(P_{\mathcal{A}}) \right) = \Theta( U(r^*))
\end{align*}
This is indeed the case for agnostic learning with bounded variation distance at each step, and also the examples in our paper over density estimation.}

\comment{
Additional observation:
To show strict optimality, we need to make two observations: $(1)$ the upper bound $U(\cdot)$ could not be tight, (2) we need to consider a broader family of empirical distribution, and not only uniform windows. For $(1)$, If we focus on the setting of evaluating the sup over a set of functions, we can prove a lower bound on the expected distance that is $\gtrsim S(r) + D(r)$ whenever the sample complexity is tight. In this case, the upper bound $U(\cdot)$ is tight up to constants. For $(2)$, we can show by using the previous paper that whenever the error can be additive (i.e., the distance can increase $\Delta$ at each step), the optimal weighting of the previous samples is up to constant close with respect to picking an optimal uniform weighting of the past.  }

\fi




